Monitoring the Top-m Aggregation in a Sliding Window of Spatial Queries

In this paper, we propose and study the problem of top-m rank aggregation of spatial objects in streaming queries, where, given a set of objects O, a stream of spatial queries (kNN or range), the goal is to report m objects with the highest aggregate rank. The rank of an object w.r.t. an individual query is computed based on its distance from the query location, and the aggregate rank is computed from all of the individual rank orderings. Solutions to this fundamental problem can be used to monitor the popularity of spatial objects, which in turn can provide new analytical tools for spatial data. Our work draws inspiration from three different domains: rank aggregation, continuous queries and spatial databases. To the best of our knowledge, there is no prior work that considers all three problem domains in a single context. Our problem is different from the classical rank aggregation problem in the way that the rank of spatial objects are dependent on streaming queries whose locations are not known a priori, and is different from the problem of continuous spatial queries because new query locations can arrive in any region, but do not move. In order to solve this problem, we show how to upper and lower bound the rank of an object for any unseen query. Then we propose an approximation solution to continuously monitor the top-m objects efficiently, for which we design an Inverted Rank File (IRF) index to guarantee the error bound of the solution. In particular, we propose the notion of safe ranking to determine whether the current result is still valid or not when new queries arrive, and propose the notion of validation objects to limit the number of objects to update in the top-m results. We also propose an exact solution for applications where an approximate solution is not sufficient. Last, we conduct extensive experiments to verify the efficiency and effectiveness of our solutions.

==> block-gain.tex <==
\myparagraph{Block-level gain computation}
Given a block $b$ from the rank list of $qn$, the block level gain $\blkgain$ is an overestimation of the gain of the objects $o \in b$, i.e., $\blkgain \ge \objgain$. As the gain is maximized when the difference between $\ac(\ar(o,qn))$ and
$\ac(\ar(o,qo))$ is maximum, therefore we present a technique to compute $\blkgain$ by finding (i) a lower bound estimation of the rank of any object $o \in b$ for  
$qn$, namely $\LBR(b,qn)$, where, $\LBR(b,qn) \le \ar(o,qn)$, and (ii) an upper bound estimation of the rank that any object $o
\in b$ can have for $qo$, denoted as $\UBR(b,qo)$, such that $\ar(o,qo) \le \UBR(b,qo)$. 



Since the objects are sorted in ascending order of their lower bound
ranks in our \irr index, the lower bound rank of the first entry of $b$ is implicitly
$\LBR(b,qn)$.
%$$
%LBR(b,qn) = LR(o,qn), \mbox{o is first(b)}
%$$
Here, $\forall o \in b, \LBR(b,qn) \le \LR(o,qn)$ holds by definition. 

Next, for the same block $b$ of the rank list of $qn$, we want to find the maximum rank $\UBR(b,qo)$ that any object $o \in b$ can have for $qo$. To achieve this, a block $b^\prime$ is found such that all of the objects $o \in b$ are guaranteed to be in the rank list of $qo$ before $b^\prime$. As the objects are sorted by $\LR(o,c_{qo})$ in the rank list of $c_{qo}$, so the $\LR(o^{\prime},c_{qo})$ is guaranteed to be greater than that
of any object in $b^\prime$, where $o^{\prime}$ is the first entry of $b^\prime$. Therefore,  $\LR(o^{\prime},qo)$ is taken as the upper bound estimation, $\UBR(b,qo)$. 
%If $o^{\prime}$ does not satisfy the query constraint, $\constraint(qo)$, then $\ac(\UBR(b,qo))$ is considered as zero. 


%\begin{equation}\label{eqn:ubr}
%UBR(b,qo) = LR(o^{\prime},qo), o^{\prime} \mbox{ is first} (b^{\prime})
%\end{equation}
For a tight estimation of $\UBR(b,qo)$, the block $b^\prime$ with the smallest $\LR(o^{\prime},qo)$ must be found.
As the objects and blocks of a rank list are sorted by the minimum
Euclidean distance from the corresponding cell
(Section~\ref{sec:index}), and $\forall o \in b,$ $\mindist(o,c_{qo}) \le \maxdist(b,c_{qo})$, a binary search over
the blocks of the rank list of $qo$ is performed to find the first
position of the block $b^{\prime}$ where $\maxdist(b,c_{qo}) \le \mindist(b^{\prime},c_{qo})$. The $\maxdist(b,c_{qo})$ is computed as the maximum Euclidean distance between the minimum bounding rectangle of the objects $o \in b$ and cell $c_{qo}$.  

\begin{example}
Computing the block gain is explained with the example shown in
Figure~\ref{fig:index}.
Let $c_1$ and $c_2$ be the cell where query $qn$ and $qo$ arrive
respectively.
Assume that the constraint on both queries are satisfied by all the objects for ease of explanation.
Let $b = \langle (o_4,3), (o_5,4) \rangle$ be the block of the
rank list of $qn$ currently under consideration.
Here, $\aLBR(b,qn) = 3$, which is the lower bound of the first entry
of $b$.
Let $\maxdist(b,c_2) = 14$.
Now, as the objects in the rank list of $c_2$ are sorted by
minimum Euclidean distance from $c_2$, a binary search is
performed with the value $14$ over the $\mindist$ of the blocks in
$c_2$.
Here, we get $b^\prime = \langle (o_6,6), (o_8,6) \rangle$, as
$\mindist(b^\prime,c_2) = 18$, which is the smallest value of
$\mindist$ greater than $14$.
So, $\aUBR(b,qo) = 6$ is the lower bound rank of the first entry of
$b^\prime$.
\end{example}

%As $\forall o \in b,$ $\mindist(o,c_{qo}) \le \maxdist(b,c_{qo})$,and all of the objects are in sorted order by $\mindist(o,c_{qo})$ in therank list, therefore all of the objects $o \in b$ are guaranteed to be found in the rank list of $qo$ before $b^\prime$.

%\shane{I think the notation has seriously gotten away from you again. Why can't all of the various upper and lower block / object bounds be defined as a function of $\rank$ or $\ar$? Is $\gain$ a function or a variable? It seems to be both. This seems to be happening to $\rho$ and $\rank$ too ...}



==> tbl-error.tex <==
\begin{table*}[t]
\centering
\caption{Percentage of result overlap for varying $m$}
%\vspace{-8pt}
\label{table:overlap}
\begin{small}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline

{\backslashbox{$m$}{Depth $k$}} & 10 & 20	& 30 & 	40	& 50	& 60 & 	70	& 75 &	80	& 90	& 100 &	150 &	200\\
\hline
%$1$ & 0 &	0	& 0	& 0	& 0	& 0.02	& 0.02	& 0.04	& 0.04	& 0.04	& 0.04	& 53.09	& 99.61\\
%$5$ & 0	& 0	& 0	& 2.89& 13.57	& 32.50	& 44.90	& 47.94	& 48.80	& 48.88	& 48.88	& 58.53	& 68.06\\
$10$ & 0	& 0.89	& 8.58	& 22.39	& 43.06& 58.99 & 	76.15	& 83.03& 86.37	& 90.13	& 90.77	& 91.13	& 91.62\\
%$20$ & 0.29	& 1.83& 7.59	& 12.02	& 12.86	& 13.06	& 15.06	& 17.76	& 22.25	& 34.55	& 43.07	& 50.98 & 58.96\\
$50$ & 10.46	 & 46.94	& 71.47	& 88.90	& 95.51	& 97.72& 99.18	& 99.47	& 99.61	& 99.67	& 99.67	& 99.70	& 99.71 \\
$100$ & 6.54	& 32.53	& 62.61	& 83.99	& 94.30	& 98.32	& 99.15	& 99.37	& 99.50& 99.58	& 99.58	& 99.59	& 99.60\\
\hline
\end{tabular}
\end{small}
\end{table*} 


==> tbl-error_foursq.tex <==
\begin{table*}[t]
\centering
\caption{Percentage of result overlap for varying $m$}
%\vspace{-8pt}
\label{table:overlap}
\begin{small}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline

{\backslashbox{$m$}{Depth $k$}} & 10 & 20	& 30 & 	40	& 50	& 60 & 	70	& 75 &	80	& 90	& 100 &	150 &	200\\
\hline
%$1$ & 0 &	0	& 0	& 0	& 0	& 0.02	& 0.02	& 0.04	& 0.04	& 0.04	& 0.04	& 53.09	& 99.61\\
%$5$ & 0	& 0	& 0	& 2.89& 13.57	& 32.50	& 44.90	& 47.94	& 48.80	& 48.88	& 48.88	& 58.53	& 68.06\\
$10$ & 0.02	& 0.05	& 0.14	& 0.34	& 0.72 & 1.42 & 	2.20	& 2.62 & 3.02	& 3.80	& 4.74	& 7.67	& 8.70\\ 
%$20$ & 0.29	& 1.83& 7.59	& 12.02	& 12.86	& 13.06	& 15.06	& 17.76	& 22.25	& 34.55	& 43.07	& 50.98 & 58.96\\
$50$ & 0.04	 & 0.11	& 0.39	& 1.02	& 1.86	& 3.27& 5.40	& 6.63	& 8.04	& 11.13	& 14.40	& 26.29	& 29.51 \\
$100$ & 0.07	& 0.59	& 1.82	& 5.31	& 10.28	& 19.36	& 30.32	& 36.37	& 43.34& 56.44	& 66.67	& 93.63	& 97.41\\
\hline
\end{tabular}
\end{small}
\end{table*} 




 

==> tbl-index_size.tex <==
\begin{table}[h]
\caption{Index size}
\vspace{-8pt}
\centering
\begin{tabular}{lrr}
\toprule
{\bfseries $\epsilon$} & {\bfseries Aus} & {\bfseries Foursq}\\
\midrule
$1$ &  $7.4$ GB & $19.5$ GB \\
$2$ &  $7.4$ GB & $17.2$ GB\\
$3$ &  $4.1$ GB & $17$ GB \\
$4$ &  $3.8$ GB & $14.2$ GB\\
$5$ &  $3.5$ GB & $13$ GB \\
\bottomrule
\end{tabular}
\label{table:size}
%\vspace{-10pt}
\end{table}



==> tbl-ratio_ep.tex <==
\begin{table}[h]
\centering
\caption{Approximation ratio for varying $\epsilon$}
%\vspace{-8pt}
\label{table:ratio_ep}
\begin{small}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline

\multicolumn{2}{|c|}{\backslashbox{Dataset}{$\epsilon$}} & 1 & 2 & 3 & 4 & 5\\
\hline
\multirow{2}{*}{\Auss} & $U$ & 1.26 & 1.27 & 1.57 & 2.17 & 2.96\\
\cline{2-7}
& $S$ & 1.19 & 1.43 & 2.14 & 2.92 &3.13 \\
\hline
\multicolumn{2}{|c|}{\Foursq}  & 2.90 & 3.22 & 3.49 & 4.15 & 5.53  \\


\hline

\end{tabular}
\end{small}
\end{table} 




